An Entropic Approach To Classical Density Functional Theory

The classical Density Functional Theory (DFT) is introduced as an application of entropic inference for inhomogeneous fluids at thermal equilibrium. It is shown that entropic inference reproduces the variational principle of DFT when information about expected density of particles is imposed. This process introduces an intermediate family of trial density-parametrized probability distributions, and consequently an intermediate entropy, from which the preferred one is found using the method of Maximum Entropy (MaxEnt). As an application, the DFT model for slowly varying density is provided, and its approximation scheme is discussed.

==> references.tex <==
\begin{thebibliography}{999}
\bibitem{kohn} Kohn, W., Hohenberg, P., Inhomogeneous electron gas. \textit{Phys. Rev.}, \textbf{1964}, \textit{136, B864}.
\bibitem{mermin} Mermin, D.,Thermal properties of inhomogeneous electron gas. \textit{Phys. Rev.} \textbf{1965}, \textit{137, A1441}.
\bibitem{ebner} Ebner, C., Saam, W.F., Stroud, D., Density-functional theory of simple classical fluids. I. surfaces. \textit{Phys. Rev. A}, \textbf{1976} \textit{14, 2264}.
\bibitem{evans79} Evans, R.,The nature of the liquid-vapor interface and other topic in statistical mechanics of non uniform, classical fluids. \textit{Advances in Physics} \textbf{1979}, \textit{28-2, 143-200}. 
\bibitem{Jaynes1} Jaynes, E.T. Information theory and statistical mechanics. \textit{Phys. Rev.}, \textbf{1957}, \textit{106, 620}. 
\bibitem{Jaynes2} Jaynes, E.T. Information theory and statistical mechanics II. \textit{Phys. Rev.} \textbf{1957}, \textit{108, 171}.
\bibitem{wdws} Jaynes, E.T., Where do we stand on maximum entropy?. \textit{The Maximum Entropy Principle ed. by R. D. Levine and M. Tribus (MITPress);} \textbf{1979}; and at \url{http://bayes.wustl.edu}.
\bibitem{psm} Jaynes, E.T. Predictive statistical mechanics. \textit{in Frontiers of Nonequilibrium Statistical Physics, G.T. Moore and M.O. Scully (eds.)(Plenum Press, New York)}, \textbf{1986}; and at \url{http://bayes.wustl.edu}.
\bibitem{entropicphysics} Caticha, A., Entropic physics, probability, entropy, and The foundations of physics.  \textit{Available online} \textbf{accessed on 12 April 2021}: \url{https://www.albany.edu/physics/faculty/ariel-caticha}.
\bibitem{rajeev} Rajeev, S.G., A Hamilton-Jacobi formalism for thermodynamics. \textit{Annals of Physics}, \textbf{323-9, 2265-2285}; and at \url{https://arxiv.org/pdf/0711.4319.pdf}.
\bibitem{HSTh} Balian, R., Valentin, P., Hamiltonian structure of thermodynamics with gauge. \textit{Eur. Phys. J. B} \textbf{2001} \textit{21, 269–282}; and at \url{https://arxiv.org/pdf/cond-mat/0007292.pdf}.
\bibitem{catichatseng} Caticha, A.,Tseng, C., Using relative entropy to find optimal approximations: an application to simple fluids. \textit{Physica A} \textbf{2008}, \textit{387, 6759}; and at \url{http://arxiv.org/abs/0808.4160v1}.
\bibitem{18} Toxvaerd, S., Perturbation theory for nonuniform fluids: surface tension, \textit{J. Chem. Phys.}, \textbf{1971} 55, 3116.
\bibitem{19} Singh, Y., and Abraham, F. F., Structure and thermodynamics of the liquid–vapor interface. \textit{J. Chem. Phys.}, \textbf{1977} \textit{67,537}.
\bibitem{22} Hansen, J-P., McDonald, I.R., Theory of simple liquids. \textit{Academic Press}, \textbf{1976}.
\bibitem{marconi1} Marconi U.M.B., Tarazona, P.,  Dynamic density functional theory of fluids. \textit{J. Chem. Phys.} \textbf{1999}, \textit{110, 8032}.
\bibitem{caliber} Jaynes, E.T., The minimum entropy production principle. \textit{Ann. Rev. Phys. Chem.}, \textbf{1980} \textit{31,579-601}. 
\bibitem{tarazona}Tarazona, P., Free-energy density functional for hard spheres. \textit{Phys. Rev. A}, \textbf{1985}, \textit{31,2672}.
\bibitem{rosenfeld} Rosenfeld, Y., Free-energy model for the inhomogeneous hard-sphere fluid mixture and density-functional theory of freezing. \textit{Phys. Rev. Lett.}, \textbf{1989}, \textit{63,980}.
\end{thebibliography}
